The Geometric Structure of Externally Actuated Planar Locomoting Systems in Ambient Media

Robots often interact with the world via attached parts such as wheels, joints, or appendages. In many systems, these interactions, and the manner in which they lead to locomotion, can be understood using the machinery of geometric mechanics, explaining how inputs in the shape space of a robot affect motion in its configuration space and the configuration space of its environment. In this paper we consider an opposite type of locomotion, wherein robots are influenced actively by interactions with an externally forced ambient medium. We investigate two examples of externally actuated systems; one for which locomotion is governed by a principal connection, and is usually considered to possess no drift dynamics, and another for which no such connection exists, with drift inherent in its locomotion. For the driftless system, we develop geometric tools based on previously understood internally actuated versions of the system and demonstrate their use for motion planning under external actuation. For the system possessing drift, we employ nonholonomic reduction to obtain a reduced representation of the system dynamics, illustrate geometric features conducive to studying locomotion, and derive strategies for external actuation.

==> sections/swimmers.tex <==
\section{Interacting Spherical Swimmers}
We now turn to an aquatic setting with external interactions among multiple locomoting agents. Similar to the example of Fig.~\ref{fig:ellipticalSwimmer}, we will consider bodies with variable mass distribution, but limit ourselves to rigid spheres to allow for simpler interaction models. Like the robot-platform system, locomotion arises due to the underlying medium, but in this example the medium \emph{facilitates} interaction among two or more agents rather than causing locomotion directly.

\subsection{Hollow Spheres Model}
We refer to the model shown in Fig.~\ref{fig:spheres4}, which shows two spherical bodies with internal masses in an ideal fluid. The indicated axis connecting the centers of the two spheres, or line of centers, is particularly useful for approximating the motions of the two bodies. The derivation of the dynamics is done in detail by \cite{lamb1932hydrodynamics} and \cite{milne1968theoretical}; here, we briefly summarize the key points, since we want to focus on the geometric structure of the problem rather than the specific interaction model. We start with a hollow spheres model, assuming no internal masses.

From Fig.~\ref{fig:spheres4}, we see that a ``body'' frame $\{x^b,y^b\}$ can be defined and attached to one of the two spheres, just as we did in defining a body frame on the three-link robot. The difference here is that the orientation of the frame will change with the \emph{displacement} of the second sphere relative to it, so that the lateral displacement component $y^b_2$ is always zero. Thus, the frame is aligned with the line of centers connecting the two bodies. The velocities of the spheres relative to this frame are $(\dot x^b_1, \dot y^b_1)$ and $(\dot x^b_2, \dot y^b_2)$, their radii are $R_1$ and $R_2$, and their masses $m_1$ and $m_2$. The surrounding ideal fluid has density $\rho$. 

The motion of the spheres within the fluid induces a velocity potential $\phi$, which must everywhere satisfy Laplace's equation, $\nabla^2 \phi = 0$. The boundary conditions are that the fluid is at rest infinitely far away from the spheres, while the motion of the spheres leads to a flux boundary condition on the bodies' surfaces. As we showed in our previous work (\cite{dear2017control}), a useful way of approximating the latter condition is to superimpose the component corresponding to the spheres moving along the line of centers (thus ensuring that $\dot y^b_i = 0$ for both spheres) with the component corresponding to motion perpendicular to the line of centers ($\dot x^b_i = 0$). 

The boundary condition can be approximated as
\begin{equation}
-\frac{\partial}{\partial n} \phi(x^b,y^b) = \frac{x^b \dot x_1^b + y^b \dot y^b_1}{R_1} + \frac{(x^b - x^b_2)\dot x_2^b + y^b \dot y_2^b}{R_2} ,
\label{eq:bc-x}
\end{equation}
where $-\frac{\partial \phi}{\partial n}$ is the flux going into each of the sphere surfaces. This flux can be viewed as a linear combination of the velocity components of each sphere. For example, suppose that the motion of the first sphere is entirely along the line of centers ($\dot y_1^b = 0$). In that case, the flux component of the first term is maximal when $x^b = \pm R$ (the two antipodes on the equator) and minimal when $x^b = 0$ (the two poles).

A solution can be obtained for $\phi$ in the form of an infinite series using the method of image doublets (\cite{lamb1932hydrodynamics, milne1968theoretical}). The kinetic energy of the fluid is given by the integration
\begin{equation}
T_{hs} = -\frac{1}{2} \rho \int \phi \frac{\partial \phi}{\partial n} \text{ d} S_1 
-\frac{1}{2} \rho \int \phi \frac{\partial \phi}{\partial n} \text{ d} S_2 
\label{eq:integrate-energy}
\end{equation}
over the surfaces of each sphere, denoted by $S_1$ and $S_2$. The idea here is that $-\frac{\partial \phi}{\partial n}$ is the normal fluid velocity into each sphere, and $\rho \phi$ is an impulse that generates the motion. Integrating their product over both of the sphere surfaces then gives us the total kinetic energy from their motion.

Again, the full solution of $\phi$ is an infinite series whose higher-order terms can be effectively ignored, since the two spheres cannot approach arbitrarily close to each other due to their finite radii. An analytical form for the kinetic energy can be written as 
\begin{align}
T_{hs} &= \frac{1}{2} M_{1} ((\dot x^b_1)^2 + (\dot y^b_1)^2) + \frac{1}{2} M_{2} ((\dot x^b_2)^2 + (\dot y^b_2)^2) \nonumber \\
&- N \left(\dot x^b_1 \dot x^b_2 - \frac{1}{2} \dot y^b_1 \dot y^b_2 \right)
\label{eq:sphere-kin-energy}
\end{align}
where $M_i$ are the \emph{effective masses} of each swimmer and $N$ is a cross-coupling term between the two. Written up to order $(x^b_2)^{-6}$, they are
\begin{align*}
M_{i} &= m_i + \frac{2}{3} \pi \rho R_i^3 \left( 1 + \frac{3R_1^3 R_2^3}{(x^b_2)^6} \right), \quad i=1,2 ; \\
N &= 2 \pi \rho \frac{R_1^3 R_2^3}{|x^b_2|^3} .
\end{align*}
For the simulations that we perform, higher-order terms are negligible even when the spheres are adjacent to each other. The relative contributions of these terms can be computed for different model parameters, but this truncation is generally sufficient when the two spheres are of similar size.

\begin{figure}
	\centering
	\includegraphics[width=3.2in]{figures/spheres4.pdf}
	\caption{Two spherical swimmers with radii $R_1$ and $R_2$, each with an internal mass. A body frame is attached to one body and oriented along the line of centers; the distance between the two bodies is $x_2^b$. The positions of the internal masses can be expressed relative to their respective sphere centers.}
	\label{fig:spheres4}
\end{figure}

Finally, if we limit the motion of the spheres to small oscillations, we can use the results of \cite{lamb1932hydrodynamics} to simplify the dynamics. Assuming the same frequency for all velocity components, the mean value of the second-order terms in the Lagrange equations will be 0. Along the line of centers, the average forces act on the spheres in opposite directions with magnitude
\begin{equation}
F_x = 3 \pi \rho R_1^3 R_2^3 \frac{2 [\dot x^b_1 \dot x^b_2] - [\dot y^b_1 \dot y^b_2]}{(x^b_2)^4},
\label{eq:avg-force-x}
\end{equation}
where $[\dot x^b_1 \dot x^b_2]$ is the mean value of $\dot x^b_1 \dot x^b_2$ (and similarly for $[\dot y^b_1 \dot y^b_2]$). The mean of the product of two sinusoidal functions differing by a phase is positive if the phase is less than a quarter period and negative otherwise. Then if the overall numerator of Eq.~\eqref{eq:avg-force-x} is positive, the spheres experience repulsion from each another; otherwise, the spheres experience an attractive force toward each other. Although the magnitude of $F_x$ varies inversely with the spheres' distances from each other, we need not worry about $F_x$ becoming unbounded since we assume finite, rigid radii for both spheres.

Finally, there are also forces acting on the bodies \emph{perpendicular} to their line of centers. They are given as
\begin{align}
F_{y,1} &= 3\pi \rho R_1^3 R_2^3 \frac{[(\dot x_2^b - \dot x_1^b) \dot y_2^b]}{(x_2^b)^4}, \nonumber \\
F_{y,2} &= 3\pi \rho R_1^3 R_2^3 \frac{[(\dot x_2^b - \dot x_1^b) \dot y_1^b]}{(x_2^b)^4}.
\label{eq:avg-force-y}
\end{align}
Unlike the forces along the line of centers, these lateral forces do not act equally on both bodies in opposite directions. Instead, the two magnitudes will vary if $\dot y^b_2$ and $\dot y^b_1$ are different.

\subsection{Adding Internal Masses}

We now consider the presence of a small mass inside each sphere, each of which can move as an actuation mechanism for the spheres. If the masses inside swimmer 1 and swimmer 2 are $\mu_1$ and $\mu_2$, respectively, and their configurations measured from their respective sphere centers are $(\xi_{1,x},\xi_{1,y})$ and $(\xi_{2,x},\xi_{2,y})$, then their kinetic energy is
\begin{equation}
T_\mu = \frac{\mu_1}{2} ((\dot \xi_{1,x})^2 + (\dot \xi_{1,y})^2) + \frac{\mu_2}{2} ((\dot x^b_2 + \dot \xi_{2,x})^2 + (\dot \xi_{2,y})^2) . \label{eq:x-kin}
\end{equation}

The total kinetic energy of the system is then $T = T_{hs}+T_\mu$, and we can use this to obtain the updated equations of motion and description of forces on the spheres. In particular, exciting $\mu_1$ and $\mu_2$ with periodic oscillations ensures that the force contributions from $T_\mu$ have a mean value of 0, so Eqs.~\eqref{eq:avg-force-x} and \eqref{eq:avg-force-y} acting on the spheres remain unchanged.

\subsubsection{Approximating Geometric Structure}

We now recast this problem into the principal bundle formulation. We have a base space $B = \mathbb R^2 \times \mathbb R^2$ formed by all possible mass configurations $(\xi_{1,x}, \xi_{1,y}, \xi_{2,x}, \xi_{2,y})$ and a set of fibers $\mathbb R^2 \times \mathbb R^2$ defined by the positions $(x^b_1,y^b_1, x^b_2,y^b_2)$ over $B$. Because of our definition of the ``body frame,'' none of the equations derived in the previous subsection have an explicit dependence on the fiber variables, with the exception of $x_2^b$. This is thus a symmetry-breaking fiber variable, capturing the role that the distance between the two bodies plays in determing their interaction. In addition, unlike with $\theta$ for the robot-platform system, $x_2^b$ generally does not have periodic trajectories in the long term (\emph{i.e.}, the bodies may oscillate but may also displace).

In cases in which the spheres are sufficiently far away from each other, we can make the following approximation of a principal connection. Momentum conservation dictates the response of each sphere due to actuation of its own internal mass, ignoring the presence of the other sphere. This gives us a constant, diagonal \emph{mechanical connection} relating the mass velocities to the sphere's perturbation velocities as
\begin{align} 
\begin{pmatrix} \dot x_{1,k} \\ \dot y_{1,k} \\ \dot x_{2,k} \\ \dot y_{2,k} \end{pmatrix} = 
&- \begin{pmatrix} \frac{\mu_1}{\mu_1 + M_1} & 0 & 0 & 0 \\ 0 & \frac{\mu_1}{\mu_1 + M_1} & 0 & 0 \\ 
0 & 0 & \frac{\mu_2}{\mu_2 + M_2} & 0 \\ 0 & 0 & 0 & \frac{\mu_2}{\mu_2 + M_2} \end{pmatrix} \nonumber \\
&\times \begin{pmatrix} \dot \xi_{1,x} \\ \dot \xi_{1,y} \\ \dot \xi_{2,x} \\ \dot \xi_{2,y} \end{pmatrix} .
\label{eq:connection}
\end{align}
In other words, we explicitly separate each fiber component $(x^b_i, y^b_i) = (x_{i,k}, y_{i,k}) + (x_{i,d}, y_{i,d})$. The first component solely captures the kinematic, oscillatory response of the spheres due to interaction with their internal masses. The second component captures the dynamic displacement of the spheres due to their interaction with each other. 

\begin{figure}
	\centering
	\includegraphics[width=3.4in]{figures/spheres_approx.pdf}
	\caption{The attraction of two spheres in response to out-of-phase perturbations of their internal masses. Solid trajectories $x_i(t)$ are computed via the full equations of motion; the dashed $\hat{x}_i(t)$ are a sum of individual and coupled approximations.}
	\label{fig:spheres-approx}
\end{figure}

Thus, given known actuation of the internal masses, we first use Eq.~\eqref{eq:connection} to find the resultant oscillations. These are then used in a modified version of the external force from Eqs.~\eqref{eq:avg-force-x} and \eqref{eq:avg-force-y} to find the external interactions as
\begin{align}
\tilde F_x &= 3 \pi \rho R_1^3 R_2^3 \frac{2 [\dot x_{1,k} \dot x_{2,k}] - [\dot y_{1,k} \dot y_{2,k}]}{(x_{2,d})^4}, \nonumber \\
\tilde F_{y,1} &= 3\pi \rho R_1^3 R_2^3 \frac{[(\dot x_{2,k} - \dot x_{1,k}) \dot y_{2,k}]}{(x_{2,d})^4}, \nonumber \\
\tilde F_{y,2} &= 3\pi \rho R_1^3 R_2^3 \frac{[(\dot x_{2,k} - \dot x_{1,k}) \dot y_{1,k}]}{(x_{2,d})^4}.
\label{eq:avg-force-decoupled}
\end{align}
The sum of the two responses, one kinematic and one dynamic, approximates the complete motion of the system. An example simulation showing the validity of this approximation is shown in Fig.~\ref{fig:spheres-approx}. We set the parameters $\rho=1$, $R_1=R_2=2$, $m_1=m_2=0$, $\mu_1=\mu_2=5$, and command the inputs $\xi_{1,x}=\cos t$, $\xi_{2,x} = \cos(t-\frac{11\pi}{12})$. For this simulation we constrain motion to occur along the line of centers, so that $\xi_{i,y}$, $\dot y_{i,k}$, and $\tilde F_{y,i}$ are all zero.

Our first observation is that because the spheres' oscillations are nearly a half-cycle out of phase with each other, the forces on each are attractive, verifying Lamb's assertion. Furthermore, the trajectories $\hat{x_i}(t)$ obtained from superimposing the individual and coupled responses of the spheres follow very closely the actual trajectories $x_i(t)$ from the full equations of motion. They only begin to diverge around $t=90$ as the spheres nearly collide. On the other hand, if the spheres were actuated so as to repel each other, this approximation would hold throughout.

\subsubsection{A Passive Swimmer}

Rather than having control of both spheres, a more challenging problem may be that we can only directly control one of the masses, while the other sphere moves according to the known hydrodynamics. Suppose that we can control the movement of the mass $\mu_1$, while $\mu_2$ can oscillate freely due to attachment to the center of its sphere via a spring. This introduces a potential energy 
\begin{equation}
V = \frac{1}{2} k ((\xi_{2,x})^2 + (\xi_{2,y})^2)
\label{eq:potential} 
\end{equation}
where $k$ is the spring constant. The full system is now described by the Lagrangian $L = T - V$. The role of the spring in the sphere with the compliant mass, here assumed to be $\mu_2$, is to allow $\mu_2$ to continue oscillating with no direct active input. 

To produce any form of desired locomotion, a primary goal is to be able to produce either attraction or repulsion of the spheres while only commanding $\mu_1$. To do this, it is useful to analyze the transfer function of the sphere velocities as a function of the input's frequency. For simplicity, we again assume motion constrained to be along the line of centers, zeroing out all terms in the $y^b$ direction. We linearize the Euler-Lagrange equations derived from $L$ and obtain the matrices $A$ and $B$ in
\[ \dot X = A X + B \xi_{1,x} , \]
where $X = (x_1^b, x_2^b, \xi_{2,x}, \dot x_1^b, \dot x_2^b, \dot \xi_{2,x})$ comprise the states and $\xi_{1,x}$ is our input. The transfer function from $\dot x_1^b$ to $\dot x_2^b$ can then be derived as a function of the frequency of $\xi_{1,x}$.

\begin{figure}
	\centering
	\includegraphics[width=1.65in]{figures/mag_w1.pdf}
	\includegraphics[width=1.65in]{figures/phase_w1.pdf}
	\caption{Transfer function response from $\dot x_1^b$ to $\dot x_2^b$ as a function of the frequency of the input $\xi_{1,x}$. The resonant frequency of the mass $\mu_2$ is 1 rad/s, close to the frequency of peak phase offset.}
	\label{fig:bode_w1}
\end{figure}

\begin{figure}
	\centering
	\includegraphics[width=1.65in]{figures/mag_w3.pdf}
	\includegraphics[width=1.65in]{figures/phase_w3.pdf}
	\caption{Same as the previous figure, except with resonant frequency 3 rad/s. As a result, both the magnitude and phase response maxima are scaled up and shifted rightward.}
	\label{fig:bode_w3}
\end{figure}

Figs.~\ref{fig:bode_w1} and \ref{fig:bode_w3} show two instances of Bode response plots of this transfer function, both using the same parameters from the simulation of Fig.~\ref{fig:spheres-approx}. Fig.~\ref{fig:bode_w1} is the response with spring constant $k = 5$ N/m; Fig.~\ref{fig:bode_w3} has spring constant $k = 45$ N/m. The magnitude plots for each show varying but finite levels of attenuation between the amplitudes of $\dot x_1^b$ and $\dot x_2^b$, which is sensible since we only actuate $\xi_{1,x}$ directly.

The transfer function is biquadratic second-order in the form 
\[ H(s) = \frac{N_2 s^2 + N_1 s + N_0}{D_2 s^2 + D_1 s + D_0} \]
with all constants being positive, so the phase offset between $\dot x_1^b$ and $\dot x_2^b$ is close to 0 at both low and high input frequencies. This means that for most inputs, repulsion of the swimmers is the only result. However, close to the resonant frequency of the compliant mass $\omega_2 = \sqrt{k/\mu_2}$, the phase offset can become much greater than 0, allowing for attractive behavior.

The optimal input frequency can be found numerically or analytically in terms of maximizing the phase or magnitude response, and choosing one is mainly a design decision that will impact the speed at which the swimmers are attracted or repelled. Here we make a qualitative observation about how the phase response changes with respect to $\omega_\xi$. For small values of $\omega_2$, such as that of Fig.~\ref{fig:bode_w1}, the maximal phase may not be able to surpass $\frac{\pi}{4}$, so that it is impossible to produce attraction while only commanding $\xi_{1,x}$. At the limit of $\omega_2=0$, $\mu_2$ is disconnected from its encompassing sphere, leaving the latter with no mechanism to oscillate on its own.

For larger values of $\omega_2$, the peak phase also becomes larger, allowing for a greater range of inputs that can produce attraction. However, a practical limitation is that a physical actuator is bounded in how fast it can operate. As $\omega_2 \rightarrow \infty$, $\mu_2$ essentially becomes rigidly attached to its sphere, again removing the oscillatory mechanism.

\begin{figure}
	\centering
	\includegraphics[width=3.3in]{figures/attract_repel_x.pdf}
	\includegraphics[width=3.3in]{figures/attract_repel_xi.pdf}
	\caption{Input frequencies to $\xi_{1,x}$ are chosen in order to produce attractive followed by repulsive locomotion of the spheres. The second plot shows $\xi_{1,x}$ around the transition time as well as the response of the compliant mass $\mu_2$.}
	\label{fig:attract-repel}
\end{figure}

Finally, this analysis can be combined with that of the previous subsection to produce desired attractive or repulsive forces on the spheres. The input $\xi_{1,x}$ produces a known oscillatory response in $\dot x_{1,k}$ through Eq.~\eqref{eq:connection}. We can obtain the corresponding response of $\dot x_{2,k}$ through the preceding transfer function analysis. The resultant forces on each sphere can then be computed via Eq.~\eqref{eq:avg-force-decoupled}, which can subsequently be integrated to find the full system trajectories.

An example simulation is shown in Fig.~\ref{fig:attract-repel}. Here we use the parameters of the system used to derive the transfer function in Fig.~\ref{fig:bode_w3}, except with $\mu_1 = 20$ to make $x_1$ oscillate faster. Suppose we want the spheres to be first attracted toward and then later repelled from each other. We thus perturb $\mu_1$ with two different frequency inputs, the first stage at 3.2 rad/s, and the second at 2 rad/s. In the first half, $\dot x_{1,k}$ and $\dot x_{2,k}$ are a quarter cycle out of phase; in the second, they are nearly completely in phase. As expected, the spheres are first attracted and then repelled, the latter occurring following a frequency, and thus phase, change in the input.

\subsection{Simplifying Motion Primitives}
The value of the numerator terms of Eq.~\eqref{eq:avg-force-decoupled} can be arbitrarily designed by choosing the desired oscillations with the right amplitude and phase. In particular, if all oscillation components take the form
\begin{align*}
\dot x_{i,k} &= A_{x,i} \cos (\omega t - \phi_{x,i}), \\
\dot y_{i,k} &= A_{y,i} \cos (\omega t - \phi_{y,i}),
\end{align*}
then Eq.~\eqref{eq:avg-force-decoupled} can be simplified to
\begin{align}
\tilde F_x &= \frac{3 \pi \rho R_1^3 R_2^3}{(x_{2,d})^4} \Big( A_{x,1} A_{x,2} \cos(\phi_{x,1}-\phi_{x,2}) \Big. \nonumber \\ 
&\qquad\qquad\qquad \Big. - \frac{1}{2} A_{y,1} A_{y,2} \cos(\phi_{y,1}-\phi_{y,2}) \Big), \nonumber \\
\tilde F_{y,1} &= \frac{3\pi \rho R_1^3 R_2^3}{(x_{2,d})^4} \frac{A_{y,2}}{2}
\Big( A_{x,2} \cos(\phi_{x,2}-\phi_{y,2}) \Big. \nonumber \\ 
&\qquad\qquad\qquad\qquad \Big. - A_{x,1} \cos(\phi_{x,1}-\phi_{y,2}) \Big), \nonumber \\
\tilde F_{y,2} &= \frac{3\pi \rho R_1^3 R_2^3}{(x_{2,d})^4} \frac{A_{y,1}}{2}
\Big( A_{x,2} \cos(\phi_{x,2}-\phi_{y,1}) \Big. \nonumber \\ 
&\qquad\qquad\qquad\qquad \Big. - A_{x,1} \cos(\phi_{x,1}-\phi_{y,1}) \Big).
\label{eq:avg-force-algebraic}
\end{align}
These equations effectively render all of the numerators as constants, since all time dependence is eliminated. Producing a desired amount of force in the numerator term then becomes a problem of solving the above nonlinear equations for the oscillation parameters.

However, $x_{2,d}$ still appears in the denominators, generally changing the effective forces on the bodies as they locomote. This difficulty normally necessitates an integration to find the resultant trajectories of the spheres, but certain motion primitives can simplify or avoid this problem altogether. We propose three motion primitives---attraction and repulsion, parallel motion, and orbiting around their centroid. The first type has $\tilde F_x \neq 0$, $\tilde F_{y,i}=0$, and the second two types have $\tilde F_x = 0$, $\tilde F_{y,i} \neq 0$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%% begin figure %%%%%%%%%%%%%%%%%%%
\begin{figure*}[t]
	\begin{center}
		\includegraphics[width=.27\textwidth]{figures/primitive-attract.pdf}	\quad		
		\includegraphics[width=.27\textwidth]{figures/primitive-parallel.pdf} \quad
		\includegraphics[width=.4\textwidth]{figures/primitive-orbit.pdf}
	\end{center}
	\caption{The three types of motion primitives that can be easily effected using Eq.~\eqref{eq:avg-force-algebraic}. The first type, motion along the line of centers, was detailed previously and only relies on $\tilde F_x$ to change $x_{2,d}$. The other two, parallel and orbital motion, keep $x_{2,d}$ relatively constant and thus can be planned without regard to the evolution of the spheres' configurations.}
	\label{fig:spherePrimitives}
\end{figure*}
%%%%%%%%%%%%%%%% end figure %%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection{Attraction and Repulsion}
We have already shown how to induce either attraction or repulsion along the line of centers only using different phase relationships in the input oscillations, \textit{e.g.} in Fig.~\ref{fig:spheres-approx} and Fig.~\ref{fig:attract-repel}. In both cases, the $\dot y_{i,k}$ component velocities were zero, leading to zero net forces on the spheres in the $y^b$ direction. This can also be achieved if both $\dot x_{i,k}$ component velocities are zero and both $\dot y_{i,k}$ components are nonzero. In either case, we have that $\tilde F_{y,1} = \tilde F_{y,2} = 0$ and the displacement between the two spheres evolves as 
\begin{equation*}
\ddot x_{2,d} \sim (x_{2,d})^{-4}.
\end{equation*}

The numerical solution of this differential equation can then be used to inform the scaling in the numerator of the first line of Eq.~\eqref{eq:avg-force-algebraic}. For example, as $x_{2,d}$ decreases, the acceleration $\ddot x_{2,d}$ and force along the line of centers $\tilde F_x$ increases rapidly. Thus, in order to maintain a constant force, the oscillation velocities must be correspondingly reduced, which is easily done by simply scaling the inputs. The opposite would hold if $x_{2,d}$ were to increase, with the force $\tilde F_x$ dropping off very quickly.

\subsubsection{Parallel Motion}
When the spheres move parallel to each other,  $x_{2,d}$ remains constant, while $\tilde F_x = 0$ and $\tilde F_{y,1} = \tilde F_{y,2}$. The easiest way to achieve these conditions is to first ensure that $\dot y_{1,k} = \dot y_{2,k}$, leading to equal forces acting on both spheres in the direction perpendicular to the line of centers. Then to have $\tilde F_x = 0$, we can simultaneously solve this nonlinear equation (using the first line of Eq.~\eqref{eq:avg-force-algebraic}) and either of the two $\tilde F_{y,i}$ equations (since they are identical) for the desired amount of force.

\subsubsection{Orbit Around Centroid}
The last motion primitive for which Eq.~\eqref{eq:avg-force-decoupled} is useful is for the spheres to orbit their centroid, thus keeping $x_{2,d}$ constant. This type of motion allows for the relative reorientation of the two bodies, which, when combined with displacement along and perpendicular to the line of centers, leads to coverage of the entire plane. The first condition for this motion is that $\tilde F_{y,1} = -\tilde F_{y,2}$, which can be achieved if $\dot y_{1,k} = -\dot y_{2,k}$. Secondly, $\tilde F_x$ must act attractively on the spheres with the same magnitude as $\tilde F_{y,i}$. These two stipulations thus inform the space of acceptable inputs for both $\dot x_{i,k}$ and $\dot y_{i,k}$.

\subsubsection{Stitching Primitives Together}

Simulations depicting the three types of motion primitives are shown in Fig.~\ref{fig:spherePrimitives}. In each of them, the spheres start at the positions indicated by the circles, and undergo the trajectories shown in their respective colors. The overlays in red depict the mean trajectories of the spheres. Note that in all of them, we can command oscillations to the spheres so that they are able to execute their motions despite an arbitrary starting orientation. This is particularly striking in the middle figure, in which the spheres undergo parallel locomotion. The input oscillations to each sphere are not symmetric, but their overall motions are still the same since the forces in the \emph{body frame} are identical.

These three motion primitives can be concatenated in various combinations to move two bodies to any two planar locations to cover all of $\mathbb R^2$. A systematic way of doing so is as follows. Suppose we want to move the two bodies from their current \emph{inertial} locations $(x_1,y_1)$ and $(x_2,y_2)$ to two desired inertial locations $(x_1^*,y_1^*)$ and $(x_2^*,y_2^*)$. We also define the quantities
\begin{align*}
d^* &= \sqrt{(y_2^*-y_1^*)^2 + (x_2^*-x_1^*)^2}, \\
\theta^* &= \text{atan2}(y_2^*-y_1^*, x_2^*-x_1^*).
\end{align*}
Then we simply execute the following motions in order:

\begin{enumerate}
	\item Use attraction or repulsion to move the bodies along their current line of centers such that $d_{2,x} = d^*$.
	\item The bodies should then undergo an orbital motion so that their relative orientation $\theta = \theta^* \pm \frac{\pi}{2}$. The bodies are now aligned orthogonally to their desired final locations. 
	\item The bodies undergo parallel motion such that their current line of centers intersects the centroid of the desired locations. In other words,
	\begin{align*}
	\frac{1}{2}(x_1^*+x_2^*) &= x_1 + c(x_2-x_1), \\
	\frac{1}{2}(y_1^*+y_2^*) &= y_1 + c(y_2-y_1)
	\end{align*}
	for some constant $c$.
	\item Undo the orbital motion from Step 2 and align the bodies such that $\theta$ is equal to $\theta^*$.
	\item The two displacement vectors between each body and its respective final location are now parallel to each other. Thus, a final parallel movement is sufficient to finish the sequence. 
\end{enumerate}
This particular concatenation of motion primitives allow two bodies to move from any two initial positions to any two desired positions in the plane. This is of course in contrast to the case of a single spherical body by itself, which is unable to achieve any net locomotion at all. 
